Sustainable AI Processing at the Edge

Edge computing is a popular target for accelerating machine learning algorithms supporting mobile devices without requiring the communication latencies to handle them in the cloud. Edge deployments of machine learning primarily consider traditional concerns such as SWaP constraints (Size, Weight, and Power) for their installations. However, such metrics are not entirely sufficient to consider environmental impacts from computing given the significant contributions from embodied energy and carbon. In this paper we explore the tradeoffs of convolutional neural network acceleration engines for both inference and on-line training. In particular, we explore the use of processing-in-memory (PIM) approaches, mobile GPU accelerators, and recently released FPGAs, and compare them with novel Racetrack memory PIM. Replacing PIM-enabled DDR3 with Racetrack memory PIM can recover its embodied energy as quickly as 1 year. For high activity ratios, mobile GPUs can be more sustainable but have higher embodied energy to overcome compared to PIM-enabled Racetrack memory.

==> Sections/architecture.tex <==
\begin{comment}
\begin{figure*}[tbp]
    \centering
    \subfloat[CIM Extended DBC\label{fig:CIM-DBC}]{
        \includegraphics[height=1.9in,valign=t]{Figures/CIM-DBC.pdf}
        \vphantom{\includegraphics[height=2.175in,valign=t]{Figures/DBC-XDWM.pdf}}%
    } 
    \subfloat[XDWM Extended DBC\label{fig:XDWM-DBC}]{
        \includegraphics[height=2.175in,valign=t]{Figures/DBC-XDWM.pdf}
    }
    \caption{DBC extensions to support POD RACING CIM.}
    \label{fig:CIM-POD-RACING}
\end{figure*}
\end{comment}

\akj{Describe the high level memory architecture, from Banks to DBCs}
The fundamental memory architecture for DWM main memory is summarized in Fig.~\ref{fig:arch-dwm}.  We propose to leverage this basic DWM memory design with extended functionality for the POD RACING memory as shown in Fig.~\ref{fig:CIM-POD-RACING}.  First, we propose to adopt a CIM technique similar to prior work~\cite{PIRM,khan2021braininspired}.  To realize these PIM operations we extend the DBCs in some tiles with an additional access port as shown in Fig.~\ref{fig:CIM-DBC}.  

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/New_TAP_2D-akj.pdf}
    \caption{Cross DWM (XDWM) concept.}
    \label{fig:my_label}
\end{figure}


==> Sections/background.tex <==
\akj{Lead in text, mention that most of the acceleration work to date has been in CNN inference}

\subsection{Back Propagation for CNN}
\akj{Xinyi and Yue, can you please help here?}
\xz{The training of the CNN includes inference, loss back-propagation, and weight update. The training process of a basic CNN model including convolution, fully-connection, and softmax layer is shown in Figure \ref{fig:cnnbp} `Training overview'. During the inference, the activation of each layer are stored for the weight update. The loss of each activation layer  is then updated ($L1, L2, L3$) back-ordered and further being utilized in weight update. The loss is initialized based on the inference result of the last layer and then being propagated back to the first layer, in which, the loss is calculated by loss function $f$ such as Cross-entropy loss \cite{de2005tutorial}, Huber loss \cite{huber1992robust}, etc. The loss is of each activation layer $L_\#$ in the CNN is calculated based on the loss and weight of its followed layer. With the loss of each activation layer, the weight is updated per convolution layer via gradient descent method \cite{amari1993backpropagation}. The weight update can be briefly described as $Wei_{new}=Wei_{cur}-L_{rate}*Wei_{diff}$, in which, the $Wei_{diff}$ is calculated via gradient descent method with activation in the inference stage and the loss in back-propagation stage.}

\xz{\noindent{\textbf{Inference}} Inference in the training stage perform the exact same operation with the general inference which is shown in Figure \ref{fig:cnnbp} `Inference'. Each input activation channel is convolved by its corresponding weight filter and then accumulated. However, the activation of each layer needs to be stored for the weight update, which leads to extra data buffer.}

\xz{\noindent{\textbf{Loss back-propagation}} After getting the loss of last layer, the loss is propagated layer by layer until reaching the first layer of CNN model which is described in Equation. Taking Loss 1 ($L1$) as an example, when knowing the loss of activation 2 ($L2$), the steps in Equation \ref{eq:cnnloss} to calculate loss $L1$ is visualized in Figure \ref{fig:cnnbp} `Loss back-propagation'. First, the weight ($W[K][K][N][M]$) of convolution 2 is rotated 180 degree in its first and second dimension. Second, the loss $L2$ is padded by zero and then performed `depth-wise' like convolution with each of the rotated weight filter of convolution 2, in which, each $L2$ channel is convolved by its corresponding weight filter but without accumulation.  Third, the `depth-wise' convolution result is accumulated according to the channel number. In the `depth-wise' convolution, the weight kernel (rotated weight of convolution 2) convolves with its corresponding the activation channel ($L2$'s channel). By recursively performing the loss calculation, the loss of each layer can be acquired.
As a result, the operations in loss back-propagation can be descried as \textcircled{1} weight rotation, \textcircled{2} convolution, \textcircled{3} channel-wise accumulation}.

\begin{equation}
    L1[b,n,r,c] =\sum_{m=1}^{M^i}\sum_{kr'=1}^{K^i}\sum_{kc'=1}^{K^i} L2[b,m,S^i\times r+kr',S^i\times c+kc']\times W'1[n,m,kr',kc']
\label{eq:cnnloss}
\end{equation}

\xz{\noindent{\textbf{Weight update}} Weight is updated in each layer individually based on the weight, activation, and the loss of the activation. $W_{diff}$ is calculated first according to Equation \ref{eq:cnnwu}. Second, the $W_{diff}$ multiply with the learning rate $L_{rate}$ and subtract the original weight ($Wei_{new}=Wei_{cur}-L_{rate}*Wei_{diff}$). The operations to update wight 2 is visualized in Figure \ref{fig:cnnbp} `Weight update'. Firstly, $W_{diff2}$ is calculated via a `depth-wise' convolution similar to Loss back-propagation, in which, it takes the activation 1 as input and $L2$ as weight. A $W_{diff}[K][K][N][M]$ is generated which will be further multiplied with learning rate $L_{rate}$. As a result, the operations in loss back-propagation can be descried as \textcircled{1} convolution, \textcircled{2} element-wise multiplication, \textcircled{3} element-wise subtraction.}

\begin{equation}
Wei_{diff}[m,n,kr,kc] =\sum_{b=1}^{B}\sum_{r=1}^{R^i}\sum_{c=1}^{C^i} L2[b,m,r,c]\times A1[b,n,S^i\times r+kr,S^i\times c+kc]
\label{eq:cnnwu}
\end{equation}

\begin{figure*}[tbp]
\centering
\includegraphics[width=0.9 \textwidth]{Figures/BP.pdf}
\caption{CNN backward propagation and weight update. }
\label{fig:cnnbp}
\vspace{-.2in}
\end{figure*}

\subsection{CNN Acceleration for Edge Computing}

Three main types of accelerators, FPGAs, Low-power GPUs, and CIM.

\akj{Xinyi and Yue, can you please help here with FPGA and GPU works?}

\subsubsection{FPGA}
\xz{The FPGA CNN accelerators are usually specialized for a certain CNN model and working under a power consumption in Watt level. It is pre-configured and working in a fixed data flow during the run time. Such characters lead to ultimate latency performance and energy efficiency when using a FPGA accelerator to accelerate a specific CNN model. At the run time, a separated DRAM (DDR) functions as its additional large capacity buffer due to the scarce on-chip buffer. FPGA accelerators are explored in both CNN inference and training.}

\paragraph{Inference}

\paragraph{Online training with Backpropagation}

\subsubsection{Low-power GPU}
\xz{The low-power GPUs are Single Instruction Multiple Threads (SIMT) processors with similar power consumption in FPGA's. The instruction based data flow make low-power GPU a generic accelerator for CNN models at the edge in compromising the latency and energy efficiency. Similar to FPGA, low-power GPU are studied in both CNN inference and training.}

\paragraph{Inference}

\paragraph{Online training with Backpropagation}

\subsection{Compute-in-Memory}
There have been two major compute-in DRAM proposals that allow bulk-bitwise processing with some operations having been demonstrated in commercial devices~\cite{ComputeDRAM}.  Bulk-bitwise logic combines two rows ``bitwise'' with the same logic operation such that $c_i = a_i$ \texttt{OP} $b_i$.  Ambit proposed to open three DRAM rows simultaneously and use the property of the senseamp (SA) to realize bitwise logic based on a majority or minority of `1's~\cite{seshadri2017ambit}.   Opening two data rows and a control row can realize \texttt{AND} and \texttt{OR}, but the result is destructive.  RowClone~\cite{seshadri2013rowclone}, can copy rows---or their inverse using a double size dual-contact cell or DCC---to conduct the logic operation leaving the original data intact.  These primitives allow computing of $A$ \texttt{XOR} $B$ by $A$ \texttt{AND} $\overline{B}$ \texttt{OR} $\overline{A}$ \texttt{AND} $B$.  Similarly, other logic such as carry can be computed to realize arithmetic functions.

ELP$^2$IM also conducts CIM using DRAM, but instead of using a destructive three row process, it changes the pseudo-precharge state of the SA~\cite{elp2im}.  The process avoids the need for cloning rows but requires multiple comparisons to determine the final logic value.  Pinatubo uses similar approaches to memories that sense a change in resistance such as phase-change (PCM), resistive (ReRAM), and spin-transfer-torque magentic (STT-MRAM) memories.  By adjusting the SA threshold above or below $\frac{V_{DD}}{2}$, \texttt{AND} and \texttt{OR} operations can be realized by opening two rows simultaneously.  For PCM and ReRAM, Pinatubo raises endurance concerns, while for STT-MRAM the density of the memory may be insufficient for sufficiently large problem sizes.

Additional CIM approaches for emerging memories include a novel memristive memory crossbar \textit{transpose memory} called MAGIC~\cite{talati2016MAGIC}.  MAGIC has the an interesting property of operation flexibility over different rows and columns, which in practice makes it hard to program and impractical while also raising endurance concerns.  CRAM extends the magneto-tunnel junction (MTJ) for STT-MRAM with a second transistor to realize bulk-bitwise operations.  Unfortunately the density of STT-MRAM is limited by the transistor per MTJ (1T1J), adding a second transistor (2T1J) makes the already insufficiently dense memory increasing sparse.  

\subsection{Domain-Wall Memory and CIM}
There are two major drawbacks of the emerging memory technologies proposed to supplement in a tiered memory configuration or replace DRAM at the main memory level.  PCM and ReRAM boast improved densities and energy with competitive access latency to DRAM, but suffer from limited endurance.  STT-MRAM, which has improved access latency, energy, and competitive endurance compared to DRAM cannot compete on density, providing a density on the order of SRAM.  

Domain-Wall Memory, provides an alternative for tiered memory that addresses these major drawbacks.  It has the necessary density, \textit{i.e.,} between 1-4F$^2$ per cell, while not suffering from  endurance concerns.  It also has a low energy consumption of circa 0.1pJ~\cite{yu2014energy} per write and a low access latency of circa 1ns.  Furthermore, it also has received significant attention for CIM targeting CNN inference~\cite{yu2014energy,CNN_DWM,PIRM}.

\begin{figure}[tbp]
\centering
\includegraphics[width=\columnwidth]{Figures/DWMZoom-fixed.pdf}
\caption{Anatomy of a domain-wall memory nanowire. }
\label{DWMzoom}
\label{fig:nanowire}
\vspace{-.2in}
\end{figure}

Domain-wall memory is made of ferromagnetic nanowires.  Each DWM nanowire consists of many magnetic domains separated by domain walls (DWs) as shown in Fig.~\ref{DWMzoom}. Each domain has its own magnetization direction based on either in-plane (+X/-X) or perpendicular (+Z/-Z) magentic anisotropy (IMA/PMA).  Binary values are represented by the magnetization direction of each domain, either parallel/antiparallel to a fixed reference. For a planar nanowire, several domains share one/few access point(s) for read and write operations~\cite{zhang2012perpendicular}. DW motion is controlled by applying a short current pulse laterally along the nanowire governed by \texttt{SL}. Since storage elements and access devices do not have a one-to-one correspondence, a random access requires two steps to complete:
%\textcircled{1} 
\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}
{\em shift} the target domain to {\em align} it with an access port and %\textcircled{2}
\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}
apply an appropriate voltage/current like in STT-MRAM to {\em read} or {\em write} the target bit.

The blue domains are dedicated for the actual data stored in memory. The grey domains are extra-domains used to prevent data loss while shifting data. 
%into the nanowire towards the extremities.
The dark blue elements are the read or read/write access ports (APs).  Fig.~\ref{DWMzoom} contains a read-only AP that has a fixed magnetic layer, indicated in dark blue, which can be read using \texttt{RWL}.  The read/write AP is shown using shift-based writing~\cite{DWM_Tapestri} where \texttt{WWL} is opened and the direction of current flows between \texttt{BL} and \textoverline{\texttt{BL}}, and reading conducted from \textoverline{\texttt{BL}} through the fin and up through \texttt{RWL} to \texttt{GND}.

\begin{figure*}[tbp]
    \subfloat[Banks\label{fig:arch-banks}]{%
      \includegraphics[height=2in]{Figures/arch-banks.pdf}
    }
    \subfloat[Subarray\label{fig:arch-subarray}]{
      \includegraphics[height=2in]{Figures/arch-subarray.pdf}
    }
    \subfloat[Domain-Block Cluster (DBC)\label{fig:arch-dbc}]{
      \includegraphics[height=2in]{Figures/arch-dbc.pdf}
    }
\caption{DWM main-memory architecture.   Memory is organized in to banks, subarrays, and tiles.  Each tile is composed of multiple DBCs determined by DWM nanowire length.  Standard DBCs contain a single access point (AP$_0$).  %CIM-augumented DBCs contain a second access point (AP$_1$) separated from AP$_0$ by the transverse read distance (TRD).
}
\label{fig:arch-dwm}
\end{figure*}

Similar to contemporary memory technologies, DWM nanowires are grouped together to form a 2D memory array with a DRAM-inspired hierarchical organization consisting of banks, subarrays, and tiles, as shown in Fig.~\ref{fig:arch-dwm}.
%The hierarchical organization consists of banks, subarrays, and tiles, as shown in Fig.~\ref{fig:RTM_array}. 
We presume basic bank structure with $B$ banks such that there are $S$ subarrays per bank, shown for $B=32$ and $S=64$ in Fig.~\ref{fig:arch-banks}.  Each subarray is broken down into $T$ tiles shown for $T=16$ in Fig.~\ref{fig:arch-subarray}.  However, each tile is constructed from bundles of DWN nanowires grouped by $R$ nanowires ($R$ is the memory row size) and referred to as a domain-block cluster (DBC)~\cite{TapeCache,ShiftsReduce}. A DBC therefore can accommodate $D$ ($D$ is the number of blue data domains per nanowire) $R$-bit memory objects. Each memory row in a DBC is distributed across nanowires, allowing parallel access of all bits belonging to the same data row. Access ports of all $R$ nanowires in the DBC point to the domain index of all nanowires and are shifted together in a lock-step fashion. The example from Fig.~\ref{fig:arch-dbc} is shown with $D=32$ and $R=512$, the standard cache line size.  Thus each tile maintains a $512 \times 512$ shape, akin to DRAM.%size of the memory bus. 
%We assume 16 \acp{DBC} per tile, 16 tiles per subarray. Furthermore, we assume a single \ac{CIM} tile or \emph{cim-tile} per subarray, capable of performing in-\ac{RTM} computations (see Section~\ref{sec:cim}). 

The state-of-the-art technique for CIM is PIRM~\cite{PIRM}, which uses a transverse read (TR) access mode~\cite{roxy2020novel} to access the number of `1's contained in a nanowire between two access points (APs) such as the read-write AP and the read-only AP shown in Fig.~\ref{fig:nanowire}.  TR has also been successfully demonstrated for misalignment (incorrect shifting) fault tolerance~\cite{ollivier2019dsn}.  PIRM demonstrates multi-operand bulk-bitwise operations and integer/fixed-point multi-operand addition and two operand multiplication.  The number of operands are limited to the TR distance, or distance between APs for which TR can successfully distinguish the number of 1's.  PRIM the highest performing by $2-3\times$ and lowest energy of the RM-based CIM techniques for integer/fixed-point CNN inference.  It is also $4-5\times$ faster than DRAM CIM techniques which utilize ternary weights for CNN inference~\cite{dracc}.  A similar technique to PIRM was also used to accelerate high dimensional computing based on bulk bitwise operations~\cite{khan2021braininspired}.

On-line training using a gradient descent technique like back propagation is challenging for CIM techniques.  Even with ``full-precision'' CNNs using fixed-point arithmetic, back propagation may be insufficiently accurate to successfully refine (train) the models particularly those with moderate to large working sets.  In these cases, floating-point computation appears necessary for sufficient accuracy for this operation mode.  Thus, we propose POD RACING, which augments DWM CIM with floating point multiply-accumulate operations for on-line CNN training.

In the next section, we provide motivation for the needed precision of online training for CNNs to demonstrate the need for POD RACING.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Inference text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
The inference function of CNNs contain 3 main types of layers: convolution layers, pooling layers, and fully connected layers, each of which can be completed in PIRM.
\subsection{Convolution}
\newcommand{\myMatrix}[1]{\mathbf{{#1}}}

The convolution layer is the process of taking a small kernel (or weight) matrix $\myMatrix{K}$, and combining it in ``windows'' with a larger matrix $\myMatrix{I}$ representing input features, at each step multiplying the overlapping positions and accumulating the results. As an example, for $\myMatrix{I}$ and $\myMatrix{K}$ of size $N\times N$ and $3\times 3$, respectively, the convolution operation for the window at $m,p$ is:
\vspace{-.05in}
\begin{equation}
    Conv(\myMatrix{I},\myMatrix{K})(m,p)= \sum_{j=0}^{2} \sum_{t=0}^{2}  \myMatrix{K}_{j,t}*\myMatrix{I}_{m+j-1,p+t-1}
\vspace{-.05in}
\end{equation}
Prior DWM work uses full precision form for convolution~\cite{CNN_DWM}.  In full precision (8-bit) mode, to multiply two values requires adding eight partial products, which using parallel addition can be done in $O(n\log n)$ operations.   PIRM has a significant advantage using the CSA technique completing the multiplication in $O(n)$ operations.  
\end{comment}

==> Sections/motivation.tex <==
\akj{Yue (and Xinyi, Sebastien), can you please help write a quantitative discussion of the precision required for inference and how fixed-point or even ternary/binary (Sebastien from NID and DrACC) provide reasonable accuracy but that these approximations are insufficient for back propagation.  Can we also point to saying that this does not need overflow checking.}

==> Sections/mult-algo.tex <==
\algdef{SE}[VARIABLES]{Variables}{EndVariables}
    {\algorithmicvariables}
    {\algorithmicend\ \algorithmicvariables}
\algnewcommand{\algorithmicvariables}{\textbf{Global variables}}

\definecolor{forestgreen}{RGB}{34, 139, 34}
\algnewcommand{\LeftComment}[1]{\(\triangleright\)#1} % for comments alignment
\algrenewcommand{\algorithmiccomment}[1]{{\color{forestgreen}\(\triangleright\)#1}}


\begin{algorithm}[tbp]
\caption{Floating-point Multiplication}
\begin{algorithmic}[1]
\State \algorithmicvariables: $OP_A, OP_B, M, E, S$
\State  \Comment {Inputs: $OP_{A,B}$ Operands}
\State  \Comment {Outputs: $M$ = Mantissa, $E$ = Exponent, $S$ = Sign}
\State
\Function{FPMultiply}{$OP_A,OP_B$}
\State \Comment {Mask off and multiply the mantissas}
\State $M_A \gets (OP_A$ \texttt{AND} 0x7FFFFF$)$ \texttt{OR} 0x800000
\State $M_B \gets (OP_B$ \texttt{AND} 0x7FFFFF$)$ \texttt{OR} 0x800000
\State $M \gets$ \textsc{Multiply} $(M_A,M_B)$
\State $norm \gets (M$ \texttt{AND} 0x00800000$)$ \Comment{normalize if $M\geq2$}
\State \Comment{Predicated $M$ normalization shift testing $norm$}
\State $norm$ ? $M \gets M >> 1$ 
\State \Comment{Mask off, add the exponents with normalization} 
\State $E_A \gets (OP_A$ \texttt{AND} 0x7F800000$)$
\State $E_B \gets (OP_B$ \texttt{AND} 0x7F800000$)$
\State $offset \gets$ 0xC0800000 \Comment{~-127 to correct exponent}
\State $norm \gets (M$ \texttt{AND} 0x00800000$)$ \Comment{normalize if $M\geq2$}
\State \Comment{Add exponents, note overflow if $E_{31} = 1$}
\State $E \gets $ \textsc{Add}$(E_A,E_B,norm,offset,0,8,23)$
\State \Comment{Mask off and determine final sign}
\State $S_A \gets (OP_A$ \texttt{AND} 0x80000000$)$
\State $S_B \gets (OP_B$ \texttt{AND} 0x80000000$)$
\State $S \gets (S_A$ \texttt{XOR} $S_B)$
\EndFunction

\end{algorithmic}

\label{alg:fp-mult}
\end{algorithm}


\begin{algorithm}[tbp]
\caption{Integer/Fixed-point Multiply and Add~\cite{PIRM}}
\begin{algorithmic}
\State \Comment{Fixed-point multiply}
\Function{Multiply}{$M_A,M_B$}

\For{$i \gets 0:22$} \Comment{23-bit Mantissa}
    \State $P[i] \gets 0$ \Comment{Initialize Partial Product}
    \State \Comment{Predicated copy on $M_A[i]$ of $M_B << i$}
    \State $M_A[0]$ ? $P[i] \gets $\textsc{Copy} $M_B$ 
    \State $M_A \gets M_A >> 1$ \Comment{align $i+1$ with 0 position}
    \State $M_B \gets M_B << 1$ \Comment{prepare $M_B << i$} 
\EndFor
    \State \textsc{Copy} $M_B$ \Comment{24-bit is a leading 1, by FP definition}
\For{$i \gets 0:2$} 
    \State $P[3i...3i+2] \gets $ \textsc{CSA-Reduction}($P[7i..7i+6]$)
\EndFor
    \State $P[2..4] \gets $ \textsc{CSA-Reduction}($P[2..8]$,48)
    \State $M \gets $ \textsc{Add}($P[0..4]$,48)
    
\EndFunction

\State

\State \Comment{Reduce 7 operands of bit-width $w$ to a Sum ($S$), Carry ($C$), and Super Carry ($C'$)}
\Function{CSA-Reduction}{$O[0...6],w$}
    \State \Comment{Intrinsic CIM operations allowed using TR~\cite{roxy2020novel}}
    \State \Comment{All bits $i$ in width $w$ in parallel~\cite{PIRM}}
    \ForAll{$i$ in $w$}
        \State $S_i \gets O[0]_i \oplus O[1]_i \oplus ... \oplus O[6]_i$
        \State $ones_i \gets \sum_{k=0}^6 O[k]_i$
        \State $C_i \gets 2 \leq  ones_i < 4 \; \text{\texttt{OR}} \; ones_i \; \geq 6$
        \State $C'_i \gets ones_i \geq 4$
    \EndFor
    \State \Return{$S,C,C'$}
\EndFunction

\State

\State \Comment{Add 5 operands of bit-width $w$ starting at lower-bound bit $l$ (default $=0$), using parallel carry and super carry chains~\cite{PIRM}, and return the Sum ($S$)}
\Function{Add}{$O[1..5],w,l=0$}
    \State \Comment{All bits $i$ in sequence to form carry chain}
    \State \Comment{$O[0],O[6]$ reserved for $C',C$; $S$ overwrites $O[0]$}
    \State $u = l + w$
    \For{$i \gets l:u-3$}
        \State $O[0]_i \gets O[0]_i \oplus O[1]_i \oplus ... \oplus O[6]_i$
        \State $ones_i \gets \sum_{k=0}^6 O[k]_i$
        \State $O[6]_{i+1} \gets 2 \leq  ones_i < 4 \; \text{\texttt{OR}} \; ones_i \; \geq 6$
        \State $O[0]_{i+2} \gets ones_i \geq 4$
    \EndFor
    \State \Comment{Compute $S,C$ for penultimate bit, $S$ for final bit}
    \State $O[0]_{u-2} \gets O[0]_{u-2} \oplus O[1]_{u-2} \oplus ... \oplus O[6]_{u-2}$
    \State $ones_{u-2} \gets \sum_{k=0}^6 O[k]_{u-2}$
    \State $O[6]_{u-1} \gets 2 \leq  ones_{u-2} < 4 \; \text{\texttt{OR}} \; ones_{u-2} \; \geq 6$
    \State $O[0]_{u-1} \gets O[0]_{u-1} \oplus O[1]_{u-1} \oplus ... \oplus O[6]_{u-1}$
    \State \Return{$O[0]$} \Comment{$O[0]$ is the final sum}
\EndFunction

\end{algorithmic}

\label{alg:int-operations}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Extra Examples
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}


%% Training phase
\Function{HDC\_Train}{$LS, \theta$}
\State \Comment{LS: List of Lang strings for training}
    \ForAll{$L_i \in LS$}
        \State $\vec{\mathcal{L}_i} \gets \textsc{Encode(}L_i\text{)}$
        \State Store $\vec{\mathcal{L}_i}$ in AM
        % \State $count \gets 0$
    \EndFor
\State
	\Return $AM$
\EndFunction

%% Inference phase
\vspace{0.6em}
\Function{HDC\_Classify}{$L, \theta, AM$}
\State \Comment{$L$: Text string to be classified}
   \State $\vec{\mathcal{T}} \gets \textsc{Encode(}L\text{)}$
    \State $\text{LangLabel} \gets \textsc{Sim\_Check(}\vec{\mathcal{T}}\text{)}$
    % \item[]
    \State \underline{Display:} $L$ is \emph{LangLabel} language.
\EndFunction



% \If{ $T_r$}
%     \ForAll{$L_i \in LS$}
%         \State $\vec{\mathcal{L}_i} \gets \textsc{Encode(}L_i\text{)}$
%         \State Store $\vec{\mathcal{L}_i}$ in AM
%         \State $count \gets 0$
%     \EndFor
    
%     % \State $\vec{\mathcal{L}_i} \gets \vec{\mathcal{T}}$
%     % \State Store $\vec{\mathcal{L}_i}$ in AM and repeat for all remaining languages
% \Else
%     \State $\vec{\mathcal{T}} \gets \textsc{Encode(}L\text{)}$
%     \State $\text{LangLabel} \gets \textsc{Sim\_Check(}\vec{\mathcal{T}}\text{)}$
%     % \item[]
%     \Statex \underline{Classification:} 
%     \State Input text is \emph{LangLabel} language.
% \EndIf

% \item[]

%% Rotate
\vspace{0.6em}
\Function{$\rho$}{$\vec{e}$}
    \State $\vec{\eta} \gets [], \vec{\psi} \gets []$
    
    \State PG\_size $\gets \frac{dim(\vec{e})}{T}$ \hspace{1em}\Comment{$T = 512$}% (cf. Section~\ref{subsec:rtm})}
    \For{$Itr \gets 0$ to PG\_size}
        \State \Comment{Rotate left within each SA}
        \State $\vec{\eta} \gets$ \emph{rol }( $\vec{e}_{[512\cdot Itr] : [512 \cdot (Itr+1)] -1}$)\label{line:concatstart}
        \State \Comment{Concatenate rotated chunks}
        \State $\vec{\psi}_{[512\cdot Itr] : [512 \cdot (Itr+1)] -1} \gets \vec{\eta}\label{line:concatend} $%\vec{\psi} ^\frown \vec{\eta}$ 
    \EndFor
\State
	\Return $\vec{\psi}$
\EndFunction

%% Similarity search 
% \item[]
\vspace{0.5em}
\Function{Sim\_Check}{$\vec{\mathcal{T}}$}
	\ForAll{ $\vec{\mathcal{L}_i} \in AM$} %Loop to iterate through the entire text
	    \State \Comment{Implemented with TRs (cf. Sec~\ref{subsec:inference})}
        \State $d_H(\vec{\mathcal{T}}, \vec{\mathcal{L}_i}) \gets$ Hamdist$(\vec{\mathcal{T}}$, $\vec{\mathcal{L}_i})$
    \EndFor\label{alg:LoopEnd} %end of loop
    \State \Comment{Implemented at the MemControl level}
    \State $\xi = \text{argmin}_{i \in \{1,\dots,22\} }(d_H(\vec{\mathcal{T}},\vec{\mathcal{L}}_i))$
\State
	\Return $\text{Label of language class }\vec{\mathcal{L}_\xi}$
\EndFunction

%% Encoding
% \State \Comment{Common to both HDC_Train and HDC_Classify}
\Function{Encode}{String L}
\State $\vec{v_0} = \vec{v_1} = \vec{v_2} = \vec{v_3} \gets 0$
\State $N \gets 4, D \gets 8192$
\State $charCount \gets 0$
\State $counters \gets 0$ \Comment{$D$ counters in total}

    % \State\Comment{For each char in $L$, compute $\vec{\phi}$ and update $counters$}
	\ForAll{ $c_i \in L$} %Loop to iterate through the entire text
        \State $\vec{c_i} \gets \theta(c_i)$   \Comment{Read HV from IM} \label{line:copy} %\text{Fetch the HV corresponding to $c_i$ from the IM}$
        \State\Comment{Rotate HVs in the N-gram}
        %  \State $\vec{v_3} \gets \rho(\vec{v_2})$, $\vec{v_2} \gets \rho(\vec{v_1})$, $\vec{v_1} \gets \rho(\vec{v_0})$, $\vec{v_0} \gets \vec{c_i}$
        \State $\vec{v_3} \gets \rho(\vec{v_2})$\label{line:permutestart}
        \State $\vec{v_2} \gets \rho(\vec{v_1})$
        \State $\vec{v_1} \gets \rho(\vec{v_0})$\label{line:permuteend}
        \State $\vec{v_0} \gets \vec{c_i}$
        
        \State $charCount \gets charCount + 1 $
        % \vfill\null
        % \columnbreak
        \If{$charCount \ge N$}
            \State \Comment{XOR with a TR operation}
            \State $\vec{\phi} = \vec{v_0} \oplus \vec{v_1} \oplus \vec{v_2} \oplus \vec{v_3}$ \label{line:xor}
            \State \Comment{Push counters at all bit positions}
            
            \For{$Itr \gets 0 \text{ to } D$} \label{line:incstart}
                \If{$\vec{\phi}_{Itr} == 1$}
                     \State counters$_{Itr}++$
                \EndIf
            \EndFor \label{line:incend}
             
            % \State counters $\gets$ counters $ + \text{ } \vec{\phi}$
            % \Comment{Not TR Levels but XOR result.}
            % \State $V_z \gets V_z \cup \{\phi\}$
        % \Else
            % \State \textbf{continue}
        \EndIf
    \EndFor\label{alg:LoopEnd} %end of loop
    
    \State %\Comment{THR: Threshold value}
    \State \Comment{Check all counters' state against THR}
    \For{$Itr \gets 0 \text{ to } D$}\label{line:thrstart}
        \If{counters$_{Itr} > THR$}
             \State $\vec{\mathcal{T}_{Itr}} \gets 1$
             \Else
             \State $\vec{\mathcal{T}_{Itr}} \gets 0$
        \EndIf
    \EndFor \label{line:thrend}
    % \text{bitWiseMajority }(\phi, \text{ } \forall \text{ } \phi \in V_z)
\State
    \Return $\vec{\mathcal{T}}$
    \item[]
\EndFunction
\end{comment}




==> Sections/multiplication.tex <==
\input{Sections/mult-algo}
To conduct floating point multiplication the operands are separated into their main components of sign, exponent, and mantissa via masking.  Using a combination of integer arithmetic on the extracted elements we can compute floating point multiplication.  We leave the elements separated to support summation.

We show the floating point multiplication in Algorithm~\ref{alg:fp-mult}.  The algorithm presumes the 32-bit floating point standard of a 23-bit mantissa, 8-bit exponent (biased by +127) and a sign bit.  First the mantissa of each operand is masked off and allocated 64-bits  

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> old/removed-from-Micro-Mag.tex <==
In particular, convolutional neural networks (CNNs) are of particular interest, but edge implementation requires satisfying strict have been effectively mapped to FPGA-based accelerators or low-energy mobile graphics processing units (GPUs) designed to provide best possible acceleration while meeting energy requirements of these edge systems.  Computing In Memory (CIM) has also been proposed for CNN inference.  The leading DRAM technique implements two approximations, DrAcc~\cite{dracc,elp2im}, which uses ternary weight neural networks (TWNs) and NID~\cite{sim2018nid,elp2im} using binary weight neural networks (BWNs). These approximations reduce the point-wise multiplication operations to bulk bitwise operations, (\textit{e.g.,} \texttt{XNOR}), to best leverage the capabilities of these CIM techniques.




DWM is particularly suitable for CNN CIM due to its high density and endurance while providing energy and performance benefits for both storage and CNN inference at different levels of precision.  
Prior work has proposed DWM CIM techniques targeting CNN inference using fixed point precision.  DW-NN measures giant magnetoresistance (GMR) of two stacked domains to compute \texttt{XOR} and when combined with pre-charge sensing amplifier (PCSA) computes addition and applies this to computing CNN inference~\cite{yu2014energy}.  SPIM extends DWM storage with dedicated skyrmion-based computing units~\cite{CNN_DWM} to support bulk-bitwise operations also with a goal to accelerated CNN inference.  PIRM leverages a transverse access method to determine the number of `1's in multiple adjacent domains providing the foundation to conduct multi-operand bulk bitwise operations and as the fundamental capability to build addition and multiplication operations.  PIRM demonstrates facility to conduct binary, ternary, and integer/fixed-point CNN inference~\cite{PIRM}.  

CNN inference accuracy can be maintained with integer/fixed-point computation or even approximated with ternary or binary weights with sufficient accuracy.  In contrast, online training methods for feed-forward neural networks such as CNNs, using methods like back propagation to compute gradient descent, require floating point computation to maintain sufficient accuracy.  As a result edge servers have primarily focused on inference computation while online training to improve CNN accuracy has traditionally depended on large scale compute resources in the cloud.  Unfortunately, this separation of inference and training requires a significant amount of communication between edge and cloud that is impractical.

In this paper we present \textit{Precision Optimized Deep-learning} (POD) using \textit{Racetrack Arithmetic Computed In-Memory for Native Gradient-descent} (RACING).  Core to POD RACING are CIM implementations of floating-point addition and multiplication required to compute the back-propagation steps.  The POD RACING extends the memory with \textit{predication buffers} that allow \textit{high throughput mode} to be applied in combination with predication registers.  POD RACING also modify the CIM unit to decrease the logic transistor cost and speed up shifting operations. This logical shifting supports normalization functions required for floating point execution.  POD RACING also supports multi-operand addition to directly allow calculation of floating point convolution windows.

The full CNN of various workloads including on-line training implemented using DWM in POD RACING


The state-of-the-art technique for CIM is PIRM~\cite{PIRM}, which uses a transverse read (TR) access mode~\cite{roxy2020novel} to access the number of `1's contained in a nanowire between two access points (APs) such as the read-write AP and the read-only AP shown in Fig.~\ref{fig:nanowire}.  TR has also been successfully demonstrated for misalignment (incorrect shifting) fault tolerance~\cite{ollivier2019dsn}.  PIRM demonstrates multi-operand bulk-bitwise operations and integer/fixed-point multi-operand addition and two operand multiplication.  The number of operands are limited to the TR distance, or distance between APs for which TR can successfully distinguish the number of 1's.  PRIM the highest performing by $2-3\times$ and lowest energy of the RM-based CIM techniques for integer/fixed-point CNN inference.  It is also $4-5\times$ faster than DRAM CIM techniques which utilize ternary weights for CNN inference~\cite{dracc}.  %A similar technique to PIRM was also used to accelerate high dimensional computing based on bulk bitwise operations~\cite{khan2021braininspired}.




